Navigation of a Quadratic Potential with Ellipsoidal Obstacles

Given a convex quadratic potential of which its minimum is the agent's goal and a Euclidean space populated with ellipsoidal obstacles, one can construct a Rimon-Koditschek (RK) artificial potential to navigate. Its negative gradient attracts the agent toward the goal and repels the agent away from the boundary of the obstacles. This is a popular approach to navigation problems since it can be implemented with local spatial information that is acquired during operation time. However, navigation is only successful in situations where the obstacles are not too eccentric (flat). This paper proposes a modification to gradient dynamics that allows successful navigation of an environment with a quadratic cost and ellipsoidal obstacles regardless of their eccentricity. This is accomplished by altering gradient dynamics with a Hessian correction that is intended to imitate worlds with spherical obstacles in which RK potentials are known to work. The resulting dynamics simplify by the quadratic form of the obstacles. Convergence to the goal and obstacle avoidance is established from almost every initial position (up to a set of measure one) in the free space, with mild conditions on the location of the target. Results are corroborated empirically with numerical simulations.

==> finite_number.tex <==
%!TEX root = autosam.tex

\subsection{Defining Graphs on Configurations} \label{sec:graphs}
%
In this section, we will show that the agent will only visit a finite number of obstacles. We do so by defining a graph on the configuration where the nodes represent obstacle and edges represent the ability to move from being $\varepsilon$-close from one obstacle to another. This graph will encode an ordering which will show that the agent will only visit a finite number of obstacles. Before defining the graph on the configuration we require the following lemma, stating that the space can be divided in hyperplanes which the agent can only traverse in one direction. 
%
\begin{lemma} \label{lem:boundary}
Let $\fz(x)$ be a quadratic potential as in \eqref{eqn_goal_def} and $\Hc$ be a hyperplane that does not intersect any obstacle and separates the space $\X$ into two halfspaces $\Hc^1$ and $\Hc^2$. Without loss of generality assume $x^* \in \Hc^1$. Let $n\in \reals^n$ be a unit vector normal to the hyperplane pointing toward $\Hc^2$. Then there exists $K_{1,2}$ such that for all $k > K_{1,2}$, $n^\top \dot x < 0$
\end{lemma}
\begin{proof} See Appendix-\ref{proof_lem3}
\end{proof}
%
The previous lemma is interpreted as follows. Once the agent transitions from $\Hc_2$ to $\Hc_1$, it will never be able to go back into $\Hc_2$. As such, we consider constructing a graph on the configuration which would describe the order in which an agent would visit each obstacle. 

In order to show that once the agent visits an obstacle it will never return to the same obstacle, consider the following construction of a graph on an arbitrary configuration. First, to formalize notation, consider a hyperplane $\Hc_{i,j}$ between obstacle $\Oc_i$ and $\Oc_j$. Because the obstacles are strictly convex, we know this strictly separating hyperplane exists \citep{boyd2004convex}. Let $\Hc^i$ denote the halfspace containing $\Oc_i$ and $\Hc^j$ denote the halfspace containing $\Oc_j$.  The agent's target $x^*$ is either in $\Hc^i$ or $\Hc^j$. Without loss of generality, let $x^* \in \Hc^j$. Now we can define a graph $G = (\ccalN,\ccalE)$, where the obstacles are nodes $\ccalN = \{1, \dots, m\}$, and the edges in $\ccalE$ represent the ability to move from one obstacle to the other. To place an edge between any pair of obstacles $\Oc_i, \Oc_j$, we check two conditions independently of each other:

\begin{condition} \label{cond_1} Hyperplane $\Hc_{i,j}$ exists such that $x^* \in \Hc^j.$ \end{condition} 

\begin{condition} \label{cond_2} Hyperplane $\Hc_{j,i}$ exists such that $x^* \in \Hc^i.$\end{condition}

Because there is always a hyperplane between two convex sets, at least one condition will be satisfied for every pair of obstacles. Therefore we define the graph by
\begin{equation} \label{equ:graph_def}
(i,j) \in \ccalE ~\textrm{if Condition \ref{cond_1} and not Condition \ref{cond_2}}.
\end{equation}  

%We will illustrate this with an example. Consider the environment in Fig \ref{EdgeEx} (a). Let us consider whether or not to place an edge between nodes two and three of the corresponding graph. We first consider the hyperplane $\Hc_{2,3}$ where $x^*\in \Hc^{3}$. In the figure, this is the dashed hyperplane. Because we are also able to draw a hyperplane $\Hc_{3,2}$ between the obstacles such that $x^* \in \Hc^2$, we do not put an edge between nodes two and three of the graph. By Lemma \ref{lem:boundary}, this means that with large enough $k$, the trajectory of the agent will never cross the boundaries to hit either $\Oc_2$ or $\Oc_3$, where by hit, we mean be $\varepsilon$-close.  

%The graph corresponding to the configuration is shown in Figure \ref{EdgeEx} (b). 
We interpret the graph as follows. Suppose the point agent is placed randomly on the free space. Then following \eqref{our_dynamics}, it may eventually hit one of the obstacles represented by the nodes on the graph. If it hits a leaf node at the end of the directed acyclic graph, it will not hit any other obstacle before reaching its target. If the agent hits any other node, then it can either go directly to the target or visit one of its child nodes. 
%\begin{figure}[!t]
%\centering
%\includegraphics[trim = {2.5cm, 0, 2.5cm, 0},width=.7\linewidth]{lemma2ex1c.png}
%\caption{We consider placing an edge between obstacles $\Oc_2$ and $\Oc_3$. The dashed line shows that there exists a hyperplane $\Hc_{2,3}$ with $x^*\in \Hc^3$ and the solid line shows there exists a hyperplane $\Hc_{3,2}$ with $x^*\in \Hc^2$. As such, there will be no edge placed between nodes 2 and 3 of the corresponding graph.}
%\label{EdgeEx}
%\end{figure}
%
%\begin{figure}[t!]
%\centering
%\includegraphics[trim = {2cm, 0, 2cm, 0},width=.4\linewidth]{lemma2ex2.pdf}
%\caption{The graph $G$ corresponding to the configuration in Figure \ref{EdgeEx}. }
%\label{EdgeEx_graph}
%\end{figure}

%\begin{figure}
%	\centering
%	\begin{subfigure}{0.24\textwidth} % width of left subfigure
%		\includegraphics[width=\textwidth]{lemma2ex1b.png}
%		\caption{~} % subcaption
%	\end{subfigure}
%	\hspace{-1em} % here you can insert horizontal or vertical space
%	\begin{subfigure}{0.24\textwidth} % width of right subfigure
%		\includegraphics[width=\textwidth]{lemma2ex2.pdf}
%		\caption{~} % subcaption
%	\end{subfigure}
%	\caption{We consider placing an edge between obstacles $\Oc_2$ and $\Oc_3$. The dashed line shows that there exists a hyperplane $\Hc_{2,3}$ with $x^*\in \Hc^3$ and the solid line shows there exists a hyperplane $\Hc_{3,2}$ with $x^*\in \Hc^2$. As such, there will be no edge placed between nodes 2 and 3 of the corresponding graph, shown in (b).} % caption for whole figure
%\label{EdgeEx}
%\end{figure}

% To make smaller
%\begin{figure}[!t] 
%	\centering
%	\begin{tabular}{cc}
%		\includegraphics[width = 1.5 in]{lemma2ex1c.png} &
%		\includegraphics[width = 1.5 in]{lemma2ex2.pdf}\\
%\small (a) & \small (b)
%\end{tabular}
%\caption{We consider placing an edge between obstacles $\Oc_2$ and $\Oc_3$. The dashed line shows that there exists a hyperplane $\Hc_{2,3}$ with $x^*\in \Hc^3$ and the solid line shows there exists a hyperplane $\Hc_{3,2}$ with $x^*\in \Hc^2$. As such, there will be no edge placed between nodes 2 and 3 of the corresponding graph, shown in (b).}
%\label{EdgeEx}
%\end{figure}
%

%\begin{lemma}\label{lem:break_cycles}
%Let $n$ be a unit vector which satisfies $n^\top \starx = 0$ and $n^\top (x-x_i) >0$ for some $x$ on the border of the repulsion zone $\mathcal{B}_k^i$. Then there exists a $K''_i(n)$ large enough such that for all $k > K''_i(n)$, $n^\top \dot x > 0$
%\end{lemma}
%\begin{proof} See Appendix-\ref{proof_break_cycles}
%\end{proof}
%

When the graph defined on the configuration does not have any cycles, then the agent will only visit a finite number of obstacles. %When the configuration has a cycle, which confirms that when the agent is close to the border of the obstacle, it will always move away from the center of the obstacle (see lemma \ref{lem:break_cycles}). 
For cycles to exist, it must be that the obstacles are equidistant from the objective. For an agent to visit an infinite number of obstacles in the cycle, it must go around each obstacle on the side opposite the target, which requires it to cross the center of the obstacle. We will show that when the agent is close to the border of the obstacle, it will always move away from the center of the obstacle (see lemma \ref{lem:break_cycles}) thereby guaranteeing that the agent will escape the cycle.

To conclude the proof of Theorem \ref{thm:main_result}, set $K$ to be equal to the largest of $K_i$ [c.f. Theorem \ref{thm:locally_escape}], $K^\epsilon$, $K^\epsilon_2$, and $K_{i,j}$ [c.f. Lemma \ref{lem:boundary}] over all obstacles and pairs of obstacles.

\begin{remark} \label{remark:cycles} The convergence for second order correction dynamics given in \cite{arXiv_version} holds only for configurations without cycles. Lemma \ref{lem:break_cycles} guarantees that the agent will navigate between the gap of adjacent obstacles in the cycle when the agent follows \eqref{our_dynamics}.
\end{remark}

\subsection{Proof of Theorem \ref{thm:locally_escape}}  \label{sec:local_escape}
We now show that the agent will indeed exit the $\varepsilon$-ball region. We accomplish this by defining two local Lyapunov function candidates for each obstacle; let $V_i: \mathcal{F} \to \mathbb{R}$
%
\begin{equation} \label{equ:local_lyap}
V_i(x) = \frac{1}{2} \starx^\top \nabla^2 \beta_i(x) \starx.
\end{equation}
%
We call this Lyapunov function candidate \emph{local} because it is only proper within the $\varepsilon$-ball of the local obstacle $\Oc_i$. The idea is that although the global Lyapunov function candidate may not be decreasing in the $\varepsilon$-ball region around the obstacle, the local Lyapunov function candidate $V_i(x)$ will guarantee that the agent moves around the obstacle toward the target $x^*$. To do so, we require $\dot V_i(x) \leq 0$, or where
%
\begin{equation}\label{equ:global_cond}
\begin{split}
\dot V  = \starx^\top &\nabla^2 \beta_i(x) \Big( -\beta(x) \starx\\
&+ \frac{\fz(x)}{k}\sum_{l = 1}\bar\beta_l(x)(x-x_l) \Big) 
\end{split}
\end{equation}
%
Similar to our definition of $\ccalV_k$ [c.f. \eqref{equ:def_ccalV}], we define
%
\begin{equation} \label{equ:repul_zone_def}
\begin{split}
\ccalV^i_k& := \Bigg\{ x\in \ccalB_{x^*}^c(\delta^*) \vert \\
& \beta(x) \leq \frac{\fz(x) \sum_{l =1}^m  \bar \beta_l(x)\starx^\top \nabla^2 \beta_i(x) (x-x_l) }{k \starx^\top \nabla^2\beta_i(x)\starx}\Bigg\},
\end{split}
\end{equation}
%
to be the region where the \emph{local} Lyapunov function candidate is increasing. Unlike the region $\ccalV_k$, we can guarantee that an agent which starts outside this region will never enter, and an agent which starts inside the region will always exit. This is the subject of Lemma \ref{lem:local_lyap_2}. For this reason, we refer to $\ccalV^i_k$ as the \emph{repulsion zone}. Intuitively, the repulsion zone is the area where the agent is very close to the obstacle, so the $(x-x^*)$ term in the dynamics which pulls the obstacle towards the target becomes negligible compared to the $(x-x_i)$ term which pushes the obstacle away from the obstacle. By substituting $\beta(x) =  \beta_i(x) \bar \beta_i(x)$, and using the fact that $\bar \beta_l (x) / \bar \beta_i (x) = \beta_i(x)/\beta_l(x)$, we get an equivalent, obstacle specific, expression for the repulsion zone  
%
\begin{equation} \label{equ:repul_zone_def2}
\begin{split}
&\ccalV^i_k := \Bigg\{ x\in \ccalB_{x^*}^c(\delta^*) \vert \\
& \beta_i(x) \leq\sum_{l =1}^m \frac{\fz(x)  \beta_i(x)\starx^\top \nabla^2 \beta_i(x) (x-x_l) }{k \beta_l(x) \starx^\top \nabla^2\beta_i(x)\starx}\Bigg\}.
\end{split}
\end{equation}
Because we are in the free space bounded away from the minimum, $\bar\beta_i(x)$ is bounded, therefore increasing $k$ means that $\beta_i(x)$ decreases at the rate $O(1/k)$.
%
%
Because $\nabla^2 \beta_i(x)$ is positive definite, we know that the denominator $k\starx^\top \nabla^2 \beta_i(x) \starx > 0$. Therefore, similar to $\ccalV_k$, as $k$ increases, the area of $\ccalV_k^i$ decreases (Figure \ref{fig:eps_ball}). Let us define $K^\epsilon_i$ to be such that for all $k > K_i^\epsilon$, we have $\ccalV_k^i \subset \ccalB^i_\varepsilon$ [c.f. \eqref{equ:def_B_varepsilon}].  %We call the region $\ccalB_k^i$ the \emph{repulsion zone} of obstacle $\Oc_i$ because it is in this zone where $\exi$ dominates the dynamics \eqref{our_dynamics}. 

By definition, $V_i$ is decreasing for all $x$ inside the $\varepsilon$-ball and outside the repulsion zone. This guarantees that the agent will escape the $\varepsilon$-ball region around each obstacle so long as it does not enter the repulsion zone. On the border of the repulsion zone $\ccalV_k^i$, the local Lyapunov function is constant since by definition, $\dot V_i(x)\vert_{x\in \partial \ccalV_k^i} = 0$. 

We now define the second \emph{local} Lyapunov function candidate which will both elucidate the behavior of the agent on the border of the repulsion zone as well as validate that the agent is moving away from the obstacle in this region. Let
%
\begin{equation}
\begin{split}
\tilde V_i(x) =& \max_{x'\in\ccalV_k^i}\left\{ (x'-x^*)^\top \nabla^2\beta_i(x) (x'-x^*) \right\}\\
& - \starx^\top \nabla^2\beta_i(x) \starx
\end{split}
\end{equation}
%
The following lemma establishes that the \emph{repulsion zone} acts like a barrier such that if the agent starts outside the repulsion zone, it will not enter the zone. Further, if the agent starts inside the repulsion zone, it will exit the repulsion zone.  
%
\begin{lemma}\label{lem:local_lyap_2}
	Given the dynamics \eqref{our_dynamics}, the function $\tilde V_i(x)$ is strictly decreasing on $\emph{\textbf{int}}\ccalV_k^i$ and constant on the border $\partial \ccalV_k^i$.
\end{lemma}
%
\begin{proof}
	See Appendix-\ref{proof_local_lyap_2}
\end{proof}
%
Lemma \ref{lem:local_lyap_2} confirms that by following the flow prescribed in \eqref{our_dynamics}, the agent will never collide with the obstacle. In fact, if the agent starts outside the repulsion zone, it will not enter the repulsion zone as doing so would require violating the Lyapunov function candidate $\tilde V_i(x)$. Lemma \ref{lem:local_lyap_2} also confirms that an agent which starts inside the repulsion zone will reach the border of the repulsion zone. 

We have shown that the agent will move toward $x^*$ for all $x$ in the $\varepsilon$-ball of obstacle $\Oc_i$ except for the repulsion zone. Further we have shown that it is impossible to enter the repulsion zone, and that if the agent starts inside the repulsion zone, it will reach the border of the repulsion zone. In fact, the border of the repulsion zone represents the region where both local Lyapunov function candidates $V_i$ and $\tilde V_i$ are constant. What is left to show is that the agent will exit the border of the repulsion zone. We accomplish this with the following two lemmas. The first confirms that the agent will always be moving in the direction away from the center when it is on the border of the repulsion zone. The second asserts that there is only one critical point on the border of the repulsion zone, and this critical point is an unstable equilibrium. 

\begin{lemma}\label{lem:break_cycles} Consider any point $x$ on the repulsion zone of $\Oc_i$ such that $(x-x_i)$ is not aligned with $(x-x^*)$. Let $n$ be a unit vector which lies on a hyperplane containing the points $x, x^*$, and $x_i$ such that $n^\top(x-x^*) = 0$ and $n^\top(x-x_i) = \delta(x) > 0$. Then there exists a large enough $K(x)$ such that for all $k > K(x)$, $n^\top\dot x > 0$
\end{lemma}
\begin{proof} See Appendix-\ref{proof_break_cycles}
\end{proof}
%
\begin{lemma} \label{lem:rep_zone}
	There exists a $K_i^\textrm{cp}$ such that for all $k > K_i^\textrm{cp}$, there is only one critical point on $\partial \ccalB_k^i$ and that critical point is an unstable equilibrium.
\end{lemma}
%
\begin{proof}
	See Appendix-\ref{proof_rep_zone}
\end{proof}
%
Lemmas \ref{lem:break_cycles} and \ref{lem:rep_zone} guarantee that the agent will exit the repulsion zone for almost every initial position. As soon as the agent exists the border of the repulsion zone, it will be in the region where the local Lyapunov function candidate $V_i$ is decreasing, meaning that returning to the repulsion zone is impossible. 


Select $K_i = \max\{K_i^\epsilon, K_i^\textrm{cp}\}$ to complete the proof.
%
%
%We also characterize the region where the global Lyapunov function is increasing specifically due to the repulsion from obstacle $\Oc_i$ to be the intersection of $\ccalB_\varepsilon^i$ defined in \eqref{equ:def_B_varepsilon} and $\ccalV_{K^\epsilon}(\delta)$ defined in \eqref{equ:def_ccalV}
%%
%\begin{equation} \label{yellowregion}
%V^i := \ccalV_{K^\epsilon}(\delta) \cap \ccalB_\varepsilon^i.
%\end{equation}
%%
%A visualization of these zones is shown in Figure \ref{fig:zone_vis} for reference.
%%
%\begin{figure}[!t] 
%\centering
%\includegraphics[width = 3 in]{zone_visualization2.png} 
%\caption{The obstacle is shown in black. The $\varepsilon$-ball around obstacle is shown by the black curve defines the region $\ccalB_\epsilon^i$ from \eqref{equ:def_B_varepsilon}. The repulsion zone defined in \eqref{equ:repul_zone_def2} is shown in blue and the region where the global Lyapunov function is increasing defined by \eqref{yellowregion} is shown in yellow. The idea is that $k$ should be selected large enough so that the regions are contained in the epsilon ball. Once inside the epsilon ball, the Local Lyapunov function guarantees that the agent will exit the $\varepsilon$-ball  to return to the region where the global Lyapunov function is decreasing.  } 
%\label{fig:zone_vis}
%\end{figure}
%%
%We now present two lemmas which formalizes the characteristics of the repulsion zone.
%%
%\begin{lemma}\label{lem:repulsion_zone}
%There exists a $K'_i$ such that for all $k > K'_i$, if the starting point $x_0$ is not in the set $\ccalB_k^i$. Then for all $t \in [0,\infty)$, $x(t) \notin \ccalB_i$. 
%\end{lemma}
%%
%\begin{proof} See Appendix-\ref{proof_lem1}.
%\end{proof}
%%
%\begin{lemma}\label{lem:repulsion_zone2}
%If $x_0 \in \ccalB_k^i$, then there exists a $t^*$ such that for all $t > t^*$, $x(t) \notin \ccalB_k^i$.
%\end{lemma}
%%
%\begin{proof} See Appendix-\ref{proof_lem2}.
%\end{proof}
%%
%Lemma \ref{lem:repulsion_zone} confirms that by following the flow prescribed in \eqref{our_dynamics}, the agent will never collide with the obstacle. When we enter the $\varepsilon$-ball region of an obstacle $\Oc_i$, the local Lyapunov function will always be decreasing. Therefore the trajectory of the agent will exit the $\varepsilon$-ball of that obstacle. Further, Lemma \ref{lem:repulsion_zone2} confirms if we start inside the repulsion zone -- that is, close enough such that the local Lyapunov function is not decreasing, then we will eventually exit the repulsion zone. Therefore, we have shown that for all $k > K'_i$ , if the agent gets $\varepsilon$-close to any obstacle, it will eventually escape that obstacle.

%\begin{lemma} \label{lem:limit_cycles} Let $\ccalH$
%\end{lemma}
%\begin{proof} This
%\end{proof}



%The local Lyapunov function (\ref{equ:local_lyap}) evaluated at some point $x\in \F$ is proportional to the volume of an ellipsoid centered at the agent's target with the same eccentricity and orientation of the obstacle where $x$ lies on its border. 


%We have therefore shown that if the agent enters an $\varepsilon$-region of an obstacle $\Oc_i$, it will exit that region. This result holds for any bounded free space, and thus we have shown that even when the obstacle is almost flat, the dynamics make the agent maneuver around the obstacle. 

